Sentinel: Multi-Patch Transformer with Temporal and Channel Attention for Time Series Forecasting

Transformer-based time series forecasting has recently gained strong interest due to the ability of transformers to model sequential data. Most of the state-of-the-art architectures exploit either temporal or inter-channel dependencies, limiting their effectiveness in multivariate time-series forecasting where both types of dependencies are crucial. We propose Sentinel, a full transformer-based architecture composed of an encoder able to extract contextual information from the channel dimension, and a decoder designed to capture causal relations and dependencies across the temporal dimension. Additionally, we introduce a multi-patch attention mechanism, which leverages the patching process to structure the input sequence in a way that can be naturally integrated into the transformer architecture, replacing the multi-head splitting process. Extensive experiments on standard benchmarks demonstrate that Sentinel, because of its ability to "monitor" both the temporal and the inter-channel dimension, achieves better or comparable performance with respect to state-of-the-art approaches.

==> tikz_multi_patch.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,472); %set diagram left start at 0, and has height of 472

%Flowchart: Process [id:dp03759897364702702] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.2 ][dash pattern={on 1.5pt off 1.5pt}] (422,198) -- (478,198) -- (478,214) -- (422,214) -- cycle ;
%Flowchart: Process [id:dp01607589676511023] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.2 ] (422,214) -- (478,214) -- (478,230) -- (422,230) -- cycle ;
%Flowchart: Process [id:dp8352446371846705] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.2 ] (422,182) -- (478,182) -- (478,198) -- (422,198) -- cycle ;

%Flowchart: Process [id:dp7212823945442997] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.4 ][dash pattern={on 1.5pt off 1.5pt}] (420,200) -- (476,200) -- (476,216) -- (420,216) -- cycle ;
%Flowchart: Process [id:dp49897276316509576] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.4 ] (420,216) -- (476,216) -- (476,232) -- (420,232) -- cycle ;
%Flowchart: Process [id:dp9486093771432185] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.4 ] (420,184) -- (476,184) -- (476,200) -- (420,200) -- cycle ;

%Flowchart: Process [id:dp849986602348801] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.7 ][dash pattern={on 1.5pt off 1.5pt}] (418,202) -- (474,202) -- (474,218) -- (418,218) -- cycle ;
%Flowchart: Process [id:dp4505391009709785] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.7 ] (418,218) -- (474,218) -- (474,234) -- (418,234) -- cycle ;
%Flowchart: Process [id:dp9164070190596261] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.7 ] (418,186) -- (474,186) -- (474,202) -- (418,202) -- cycle ;

%Flowchart: Process [id:dp2000373181933055] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=1 ][dash pattern={on 1.5pt off 1.5pt}] (416,204) -- (472,204) -- (472,220) -- (416,220) -- cycle ;
%Flowchart: Process [id:dp9480404545981311] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=1 ] (416,220) -- (472,220) -- (472,236) -- (416,236) -- cycle ;
%Flowchart: Process [id:dp631796166407] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=1 ] (416,188) -- (472,188) -- (472,204) -- (416,204) -- cycle ;

%Flowchart: Process [id:dp9764397157966509] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.2 ][dash pattern={on 1.5pt off 1.5pt}] (422,258) -- (478,258) -- (478,274) -- (422,274) -- cycle ;
%Flowchart: Process [id:dp592049022891634] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.2 ] (422,274) -- (478,274) -- (478,290) -- (422,290) -- cycle ;
%Flowchart: Process [id:dp16157129743801435] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.2 ] (422,242) -- (478,242) -- (478,258) -- (422,258) -- cycle ;

%Flowchart: Process [id:dp9383624023115051] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.4 ][dash pattern={on 1.5pt off 1.5pt}] (420,260) -- (476,260) -- (476,276) -- (420,276) -- cycle ;
%Flowchart: Process [id:dp6399677769888155] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.4 ] (420,276) -- (476,276) -- (476,292) -- (420,292) -- cycle ;
%Flowchart: Process [id:dp33072769980721795] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.4 ] (420,244) -- (476,244) -- (476,260) -- (420,260) -- cycle ;

%Flowchart: Process [id:dp3972003824610111] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.7 ][dash pattern={on 1.5pt off 1.5pt}] (418,262) -- (474,262) -- (474,278) -- (418,278) -- cycle ;
%Flowchart: Process [id:dp003890526488311563] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.7 ] (418,278) -- (474,278) -- (474,294) -- (418,294) -- cycle ;
%Flowchart: Process [id:dp6635405777741255] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.7 ] (418,246) -- (474,246) -- (474,262) -- (418,262) -- cycle ;

%Flowchart: Process [id:dp616028647838204] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=1 ][dash pattern={on 1.5pt off 1.5pt}] (416,264) -- (472,264) -- (472,280) -- (416,280) -- cycle ;
%Flowchart: Process [id:dp2186971054466409] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=1 ] (416,280) -- (472,280) -- (472,296) -- (416,296) -- cycle ;
%Flowchart: Process [id:dp01507361679078123] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=1 ] (416,248) -- (472,248) -- (472,264) -- (416,264) -- cycle ;

%Flowchart: Process [id:dp18881217143944795] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.2 ][dash pattern={on 1.5pt off 1.5pt}] (422,318) -- (478,318) -- (478,334) -- (422,334) -- cycle ;
%Flowchart: Process [id:dp5068618429438867] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.2 ] (422,334) -- (478,334) -- (478,350) -- (422,350) -- cycle ;
%Flowchart: Process [id:dp5222300533874498] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.2 ] (422,302) -- (478,302) -- (478,318) -- (422,318) -- cycle ;

%Flowchart: Process [id:dp7809212126360199] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.4 ][dash pattern={on 1.5pt off 1.5pt}] (420,320) -- (476,320) -- (476,336) -- (420,336) -- cycle ;
%Flowchart: Process [id:dp6770621269826098] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.4 ] (420,336) -- (476,336) -- (476,352) -- (420,352) -- cycle ;
%Flowchart: Process [id:dp2577942811321452] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.4 ] (420,304) -- (476,304) -- (476,320) -- (420,320) -- cycle ;

%Flowchart: Process [id:dp5283942817149263] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.7 ][dash pattern={on 1.5pt off 1.5pt}] (418,322) -- (474,322) -- (474,338) -- (418,338) -- cycle ;
%Flowchart: Process [id:dp1337503327198375] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.7 ] (418,338) -- (474,338) -- (474,354) -- (418,354) -- cycle ;
%Flowchart: Process [id:dp12370809671603666] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.7 ] (418,306) -- (474,306) -- (474,322) -- (418,322) -- cycle ;

%Flowchart: Process [id:dp9134343102235396] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=1 ][dash pattern={on 1.5pt off 1.5pt}] (416,324) -- (472,324) -- (472,340) -- (416,340) -- cycle ;
%Flowchart: Process [id:dp8391485911624061] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=1 ] (416,340) -- (472,340) -- (472,356) -- (416,356) -- cycle ;
%Flowchart: Process [id:dp1420003303184676] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=1 ] (416,308) -- (472,308) -- (472,324) -- (416,324) -- cycle ;

%Straight Lines [id:da7870830330592657] 
\draw    (472,364) -- (484.59,351.41) ;
\draw [shift={(486,350)}, rotate = 135] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Straight Lines [id:da14574085469531384] 
\draw    (380,212) -- (398,212) ;
\draw [shift={(400,212)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Straight Lines [id:da35384055572925455] 
\draw    (380,272) -- (398,272) ;
\draw [shift={(400,272)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Straight Lines [id:da6126906736817161] 
\draw    (380,332) -- (398,332) ;
\draw [shift={(400,332)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Flowchart: Process [id:dp8663218794262189] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.6 ][dash pattern={on 1.5pt off 1.5pt}] (132,264) -- (188,264) -- (188,280) -- (132,280) -- cycle ;
%Flowchart: Process [id:dp28587897932085693] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.6 ] (132,280) -- (188,280) -- (188,296) -- (132,296) -- cycle ;
%Flowchart: Process [id:dp2061630041267437] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.6 ] (132,248) -- (188,248) -- (188,264) -- (132,264) -- cycle ;

%Flowchart: Process [id:dp8276990067547745] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.6 ][dash pattern={on 1.5pt off 1.5pt}] (160,264) -- (216,264) -- (216,280) -- (160,280) -- cycle ;
%Flowchart: Process [id:dp2298833785572132] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.6 ] (160,280) -- (216,280) -- (216,296) -- (160,296) -- cycle ;
%Flowchart: Process [id:dp8811433355719955] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.6 ] (160,248) -- (216,248) -- (216,264) -- (160,264) -- cycle ;

%Flowchart: Process [id:dp2530399073984826] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.6 ][dash pattern={on 1.5pt off 1.5pt}] (244,264) -- (300,264) -- (300,280) -- (244,280) -- cycle ;
%Flowchart: Process [id:dp3863056991756202] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.6 ] (244,280) -- (300,280) -- (300,296) -- (244,296) -- cycle ;
%Flowchart: Process [id:dp4634205496431365] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.6 ] (244,248) -- (300,248) -- (300,264) -- (244,264) -- cycle ;

%Flowchart: Process [id:dp681902679559504] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.6 ][dash pattern={on 1.5pt off 1.5pt}] (244,264) -- (272,264) -- (272,280) -- (244,280) -- cycle ;
%Flowchart: Process [id:dp1772869965677455] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.6 ] (244,280) -- (272,280) -- (272,296) -- (244,296) -- cycle ;
%Flowchart: Process [id:dp14701076146181458] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.6 ] (244,248) -- (272,248) -- (272,264) -- (244,264) -- cycle ;

%Flowchart: Process [id:dp37213654533151264] 
\draw  [fill={rgb, 255:red, 219; green, 181; blue, 181 }  ,fill opacity=0.6 ] (132,355.24) -- (300,355.24) -- (300,370.86) -- (132,370.86) -- cycle ;
%Flowchart: Process [id:dp6922072727799429] 
\draw  [fill={rgb, 255:red, 195; green, 152; blue, 152 }  ,fill opacity=0.6 ][dash pattern={on 1.5pt off 1.5pt}] (132,339.62) -- (300,339.62) -- (300,355.24) -- (132,355.24) -- cycle ;
%Flowchart: Process [id:dp9257015001687192] 
\draw  [fill={rgb, 255:red, 152; green, 112; blue, 112 }  ,fill opacity=0.6 ] (132,324) -- (300,324) -- (300,339.62) -- (132,339.62) -- cycle ;
%Straight Lines [id:da9470986946173057] 
\draw    (116,328) -- (116,294) ;
\draw [shift={(116,292)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Shape: Rectangle [id:dp039564976787289874] 
\draw  [fill={rgb, 255:red, 241; green, 229; blue, 209 }  ,fill opacity=1 ] (356,188) -- (356,356) -- (340,356) -- (340,188) -- cycle ;
%Straight Lines [id:da7829879746504618] 
\draw    (308,272) -- (330,272) ;
\draw [shift={(332,272)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Shape: Rectangle [id:dp7054144076886071] 
\draw  [fill={rgb, 255:red, 182; green, 199; blue, 170 }  ,fill opacity=1 ] (564,188) -- (564,356) -- (512,356) -- (512,188) -- cycle ;
%Straight Lines [id:da06405574729490704] 
\draw    (484,212) -- (502,212) ;
\draw [shift={(504,212)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Straight Lines [id:da05145789175603155] 
\draw    (484,272) -- (502,272) ;
\draw [shift={(504,272)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Straight Lines [id:da9269953891747664] 
\draw    (484,332) -- (502,332) ;
\draw [shift={(504,332)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Shape: Brace [id:dp0909625861941239] 
\draw   (299.57,239.86) .. controls (299.59,235.19) and (297.27,232.85) .. (292.6,232.83) -- (225.88,232.6) .. controls (219.21,232.57) and (215.89,230.23) .. (215.91,225.57) .. controls (215.89,230.23) and (212.55,232.55) .. (205.88,232.53)(208.88,232.54) -- (139.17,232.3) .. controls (134.5,232.28) and (132.16,234.6) .. (132.14,239.27) ;

% Text Node
\draw (160,364.03) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{38.08pt}\setlength\topsep{0pt}
$\displaystyle x_{0,0}$
\end{minipage}};
% Text Node
\draw (160,332.79) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{38.08pt}\setlength\topsep{0pt}
$\displaystyle x_{0,C}$
\end{minipage}};
% Text Node
\draw (272,332.79) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{38.08pt}\setlength\topsep{0pt}
\begin{flushright}
$\displaystyle x_{L,C}$
\end{flushright}

\end{minipage}};
% Text Node
\draw (272.5,363.54) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{38.08pt}\setlength\topsep{0pt}
\begin{flushright}
$\displaystyle x_{L,0}$
\end{flushright}

\end{minipage}};
% Text Node
\draw (216,348.41) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{108.8pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (216,364.03) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{108.8pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (216,332.79) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{108.8pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (86,348) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{57.12pt}\setlength\topsep{0pt}
\begin{flushright}
$\displaystyle X\in \mathbb{R}^{L\times C}$
\end{flushright}

\end{minipage}};
% Text Node
\draw (87.5,312) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{33.14pt}\setlength\topsep{0pt}
\begin{flushright}
Patching
\end{flushright}

\end{minipage}};
% Text Node
\draw (347,272) node  [font=\tiny,rotate=-90] [align=left] {\begin{minipage}[lt]{108.8pt}\setlength\topsep{0pt}
\begin{center}
Projection
\end{center}

\end{minipage}};
% Text Node
\draw (132,304.88) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
0
\end{center}

\end{minipage}};
% Text Node
\draw (188,304.88) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
PS
\end{center}

\end{minipage}};
% Text Node
\draw (160,304.88) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
S
\end{center}

\end{minipage}};
% Text Node
\draw (216,304.88) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{16.32pt}\setlength\topsep{0pt}
\begin{center}
PS+S
\end{center}

\end{minipage}};
% Text Node
\draw (230,273) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{19.04pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (244,304.88) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{16.32pt}\setlength\topsep{0pt}
\begin{center}
L-PS
\end{center}

\end{minipage}};
% Text Node
\draw (300,304.88) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{16.32pt}\setlength\topsep{0pt}
\begin{center}
PS
\end{center}

\end{minipage}};
% Text Node
\draw (272,304.88) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{16.32pt}\setlength\topsep{0pt}
\begin{center}
PS-S
\end{center}

\end{minipage}};
% Text Node
\draw (83,272) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{61.2pt}\setlength\topsep{0pt}
\begin{flushright}
$\displaystyle X\in \mathbb{R}^{N\times C\times PS}$
\end{flushright}

\end{minipage}};
% Text Node
\draw (408,228) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
0
\end{center}

\end{minipage}};
% Text Node
\draw (408,196) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
H
\end{center}

\end{minipage}};
% Text Node
\draw (408,212) node  [font=\tiny,rotate=-90] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (408,288) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
0
\end{center}

\end{minipage}};
% Text Node
\draw (408,256) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
H
\end{center}

\end{minipage}};
% Text Node
\draw (408,272) node  [font=\tiny,rotate=-90] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (408,348) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
0
\end{center}

\end{minipage}};
% Text Node
\draw (408,316) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
H
\end{center}

\end{minipage}};
% Text Node
\draw (408,332) node  [font=\tiny,rotate=-90] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (372,212) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
Q
\end{center}

\end{minipage}};
% Text Node
\draw (372,272) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
K
\end{center}

\end{minipage}};
% Text Node
\draw (372,332) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
V
\end{center}

\end{minipage}};
% Text Node
\draw (538,272) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{35.36pt}\setlength\topsep{0pt}
\begin{center}
Scaled \\Dot-Product\\Attention
\end{center}

\end{minipage}};
% Text Node
\draw (216,220) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{114.24pt}\setlength\topsep{0pt}
\begin{center}
Patches
\end{center}

\end{minipage}};
% Text Node
\draw (485.31,363.31) node  [font=\tiny,rotate=-315] [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
N
\end{center}

\end{minipage}};


\end{tikzpicture}


